A metamaterial telescope at millimetre wavelengths

In this paper we present a novel telescope composed exclusively of thin, flat optical elements, each being a hot-pressed multi-layered structure combining the properties of a lens, its anti-reflection coating and frequency selection or filtering. We discuss the design process, from fundamental physical metamaterial properties of the single periodic cell structure to the lens concept, which constitutes the building block of the telescope design, and the iterative process that is part of the lens optimization. We provide the results of a laboratory test campaign for different telescope designs based on three-lens arrangements. Beam cuts and focus measurements both on- and off-axis are compared with models showing good agreement. We conclude that a broad-band mm-wave complete telescope system consisting entirely of metamaterial flat lenses has been built and tested, showing comparable performance with conventional state-of-the-art refractive telescopes in the same wavelength region. This new broadband design, highly efficient at frequencies between 90 and 190 GHz, offers multiple advantages. These include a $> 80\%$ weight reduction, reduced issues tied to coating-survivability at cryogenic temperatures caused by differential contraction exacerbated by non-flat surfaces, as well as a reduction in the overall number of components and mechanical mounts.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


